Learning Common Representation from RGB and Depth Images

We propose a new deep learning architecture for the tasks of semantic segmentation and depth prediction from RGB-D images. We revise the state of art based on the RGB and depth feature fusion, where both modalities are assumed to be available at train and test time. We propose a new architecture where the feature fusion is replaced with a common deep representation. Combined with an encoder-decoder type of the network, the architecture can jointly learn models for semantic segmentation and depth estimation based on their common representation. This representation, inspired by multi-view learning, offers several important advantages, such as using one modality available at test time to reconstruct the missing modality. In the RGB-D case, this enables the cross-modality scenarios, such as using depth data for semantically segmentation and the RGB images for depth estimation. We demonstrate the effectiveness of the proposed network on two publicly available RGB-D datasets. The experimental results show that the proposed method works well in both semantic segmentation and depth estimation tasks.

==> macrostm.tex <==
%Commands for references
\usepackage{xspace}

%Commands for comments
%\newcommand{\note}[1]{{\bf \it [#1]}}
\newcommand{\jjv}[1]{{\bf \color{red} [#1]}}
\newcommand{\thomas}[1]{{\bf \blue{red} [#1]}}

\newcommand{\subitem}[1]{\begin{itemize}\item #1\end{itemize}}
\newcommand{\subitemA}[1]{\begin{itemize}\item #1}
\newcommand{\subitemB}[1]{\item #1}
\newcommand{\subitemC}[1]{\item #1\end{itemize}}

% macros for todo  notes and comments
\newcommand{\todo}[1]{{\bf \color{red} TODO: #1}}
%\newcommand{\note}[1]{{\bf \color{red} NOTE: #1}}
%\newcommand{\url}[1]{{\texttt{#1}}}

%Specific macros for math symbles
\newcommand{\ka}{k\prime}
\newcommand{\ia}{i\prime}
\newcommand{\logl}{\mathcal{L}}
\newcommand{\deriv}[2]{\frac{\partial {#1}}{\partial {#2}}}
\newcommand{\minus}{\textrm{-}}
\newcommand{\plus}{\textrm{+}}
\newcommand{\T}{\top}
\newcommand{\trans}[1]{{#1}^{\T}}
\newcommand{\norm}[1]{||#1||}
\newcommand{\snorm}[1]{\norm{#1}_2^2}
\newcommand{\ind}[1]{[\![#1]\!]}
\newcommand{\hinge}[1]{[#1]_{+}}
\newcommand{\dotp}[2]{\langle #1,#2 \rangle}
\newcommand{\bigo}[1]{\mathcal{O}(#1)}
\newcommand{\kl}[2]{\mathcal{D}_{\textsc{KL}}(#1||#2)}

\newcommand{\st}{\textrm{subject to}}
\DeclareMathOperator*{\mini}{minimise}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\trace}{tr}


% General macros
\newcommand{\tabs}[2]{Tables~\ref{tab:#1}-\ref{tab:#2}}

\newenvironment{sitemize}{\vspace{-10pt}\begin{itemize}\setlength{\itemsep}{-1pt}}{\end{itemize}}
\newenvironment{senumerate}{\vspace{-10pt}\begin{enumerate}\setlength{\itemsep}{-1pt}}{\end{enumerate}}

\newlength{\mywidth}
\newlength{\myheight}
\newlength{\imgwidth}
\newlength{\imgheight}



%% Macros from Jakob Verbeek
\def\code#1{\begin{quote}{\tt #1}\end{quote}}
\def\I{{\rm I\!I}}                            % the indicator function
\def\R{{\rm I\!R}}                            % the real numbers
\def\matlab{\textsc{\small Matlab }}        % matlab add
\def\Tr#1{\textrm{Tr}\{#1\}}                % trace
\def\diag#1{\textrm{diag}\left( #1 \right)} % diag
\def\Gauss#1#2#3{\mathcal{N}\left(#1 ; #2,#3\right)}   % Gaussian density
\def\ex#1#2{\textrm{I\!E}_{#1}\!\left[#2\right]}     % expectation
\def\half{\frac{1}{2}}              % half
\def\<{\langle}
\def\>{\rangle}

\def\nn{\nonumber}

% BOLD stuff
\def\alphabold{\mbox{\boldmath $\alpha$}}
\def\betabold{\mbox{\boldmath $\beta$}}
\def\gammabold{\mbox{\boldmath $\gamma$}}
\def\mubold{\mbox{\boldmath $\mu$}}
\def\kappabold{\mbox{\boldmath $\kappa$}}
\def\epsbold{\mbox{\boldmath $\epsilon$}}
\def\thetabold{\mbox{\boldmath $\theta$}}
\def\phibold{\mbox{\boldmath $\phi$}}
\def\Upsilonbold{\mbox{\boldmath $\Upsilon$}}
\def\eye{{\bf I}}

\def\Eqs#1{Eqs.~(\ref{eq:#1})}
\def\Eq#1{Eq.~(\ref{eq:#1})}
\def\eq#1{(\ref{eq:#1})}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bea{\begin{eqnarray*}}
\def\eea{\end{eqnarray*}}

\def\fig#1{Figure~\ref{fig:#1}}
\def\tab#1{Table~\ref{tab:#1}}
\def\sect#1{Section~\ref{sec:#1}}
\def\chap#1{Chapter~\ref{chap:#1}}
\def\app#1{Appendix~\ref{app:#1}}


\newcommand{\bt}[1]{\begin{tabular}{#1}}
\newcommand{\et}{\end{tabular}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}


\def\qed{\hbox{\vrule\vbox{\hrule width .65em\vskip .65em\hrule}\vrule}}
\def\proof{\noindent\hspace{2em}{\it Proof: }}
\def\endproof{\hspace*{\fill}~\qed\par\endtrivlist\unskip}

\makeatletter
%\gdef\SetFigFont#1#2#3{%
%  \reset@font\fontsize{10}{12pt}%
%  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
%  \selectfont%
%}
\let\eqnarray@=\eqnarray \let\endeqnarray@=\endeqnarray
\def\eqnarray{\bgroup\arraycolsep=2pt\eqnarray@}
\def\endeqnarray{\endeqnarray@\egroup}
\makeatother
\def\arraystretch{1.2}
\def\em{\slshape}

\usepackage{times,amsmath,amssymb,amsbsy,xspace}
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot} 
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}

\definecolor{xturkos}{rgb}{.2039,.7373,.7294} %picked by KColorChooser, from ppt-template
\definecolor{xblue}{rgb}{.1569,.5843,.8353} %picked by KColorChooser, from ppt-template
%\definecolor{xgrey}{rgb}{.5451,.5529,.5569} %picked by KColorChooser, from ppt-template
\definecolor{xred}{rgb}{.98,.15,.15}

\def\cx{\color{xred}}
\def\cxt{\color{xturkos}}
\def\bx{\color{xblue}}
\def\gx{\color{dgreen}}
\definecolor{dgreen}{rgb}{0,0.5,0}
\definecolor{dorange}{rgb}{1,0.5,0}

\newcommand{\cbt}[1]{\textcolor{xblue}{#1}}
\newcommand{\bbf}[1]{\textcolor{xblue}{\bf #1}}
\newcommand{\rbf}[1]{\textcolor{xred}{\bf #1}}
\newcommand{\bit}[1]{\textcolor{xblue}{\em #1}}
\newcommand{\bbi}[1]{\textcolor{xblue}{\bf \em #1}}
\newcommand{\textbbf}[1]{\bbf{#1}}
\newcommand{\textblue}[1]{\textcolor{xblue}{#1}}
\newcommand{\textred}[1]{\textcolor{xred}{#1}}
%\newcommand{\positem}{\item[\checkmark]}
%\newcommand{\negitem}{\item[\rbf{$\times$}]}
\newcommand{\positem}{\item[\textblue{\ding{51}}]}
\newcommand{\negitem}{\item[\rbf{\ding{55}}]}

==> training.tex <==
%===============================================
\section{MODEL TRAINING AND OPTIMIZATION}
\label{sec:train}

% g
The encoder for all out method is a dilated ResNet101 pretrained on COCO dataset~\cite{}.
The training procedure is split in two main phases. We initially train each branch separately: the RGB-SS, DDD-SS and DDD-D branches are trained independently for 20000 iterations. We train the RGB-SS and the DDD-SS using Stochastic gradient descent with momentum 0.9 and batch size 18. We use a standard cross-entropy loss for RGB-SS; and we train the DDD-D using the smoothL1 loss, that resulted to be the most stable loss for our problem. 
We also apply weight decay 0.0005 and polynomial decay for the learning rate (base learning rate 0.00025 and power 0.9).
After this, we merge the two branches using the correlation network and we add a final convolutional module (a Classifier for the Segmentation task, and a Regressor for the Depth Estimation task).
We fine-tune all the network end-to-end freezing the encoding layers (i.e. freezing the ResNet layers) to speed-up the computations. In this second phase we use the Adam optimizer and we need to consider also an additional loss that is responsible for the projection and reconstruction task.
For the Segmentation task we also apply data augmentation, flipping and randomly rotating between [-10, 10] our inputs (RGB and Depth input are augmented randomly, but always  with the same pairwise augmentation at each step). 
The RGB images are normalized to [-0.5, +0.5] and the Depth map is normalized to [0, 1]. All inputs are resized to (512, 512).
% g

We train all the network end-to-end.
Training the encoder-decoder, softmax loss

Restating our goals more formally, given a two-view data $\bfZ = \{(\bfz_i)\}_{i=1}^N= \{(\bfx_i,\bfy_i)\} _{i=1}^N$, for each instance, ($\bfx_i,\bfy_i)$, we would like to achieve:
\begin{enumerate}
\item Minimize the self-reconstruction error, i.e., minimize the error in reconstructing
$\bfx_i$ from $\bfx_i$ and $\bfy_i$ from $\bfy_i$.
\item Minimize the cross-reconstruction error, i.e., minimize the error in reconstructing
$\bfx_i$ from $\bfy_i$ and $\bfy_i$ from $\bfx_i$
\item Maximize the correlation between the hidden representations of both views.
\end{enumerate}
We achieved this by finding the parameters $\theta = \{\bfW,\bfV,\bfW_0,\bfV_0,\bfb,\bfb_0\}$ which minimize the following objective function:
\begin{equation}
{\cal J} Z (\theta) = \sum^N_{i=1} (L(\bfz_i, g(h(\bfz_i)))+L(\bfz_i, g(h(\bfx_i)))+L(\bfz_i, g(h(\bfy_i))))-\lambda corr(h(\bfX), h(\bfY)),
\end{equation}
\noindent where 
\begin{itemize}
\item $L$ is the reconstruction error, 
\item $\lambda$ is the scaling parameter to scale the fourth term with respect to the remaining three terms, 
\item $h(\bfX)$ and $h(\bfY)$ are the mean vectors for the hidden representations of the first/second views.
\end{itemize}
 
If all dimensions in the input data take binary values then we use cross-entropy as the reconstruction error otherwise we use squared error loss as the reconstruction error. For simplicity, we use the shorthands $h(\bfx_i)$ and $h(\bfy_i)$ to note the
representations $h((\bfx_i,0))$ and $h((0,\bfy_i))$ that are based only on a single view. For each
data point with 2 views $\bfx$ and $\bfy$, $h(\bfx_i)$ just means that we are computing the hidden 
representation using only the $\bfx$-view. Or in other words, in equation 
$h(\bfz) = f(\bfW \bfx+ \bfV \bfy+\bfb)$, we set $\bfy=0$. So, $h(\bfx) = f(\bfW \bfx+ \bfb)$. 
%$h(\bfx) = h(\bfx, 0)$ is notation we are defining. 
$h(\bfz), h(\bfx)$ and $h(\bfy)$ are certainly not guarantied to be identical,
though training will gain in making them that way, because of the various reconstruction terms. The correlation term in the objective function is calculated considering the hidden representation as a random vector. In words, the objective function decomposes as follows. The first term is the usual
autoencoder objective function which helps in learning meaningful hidden representations. The second term ensures that both views can be predicted from the shared representation of the first view alone. The third term ensures that both views can be predicted from the shared representation of the second view alone. The fourth term interacts with the other objectives to make sure that the hidden representations are highly correlated.

%------------------------------------------------
\subsection{Implementation}
\label{ssec:implementation}

The proposed architecture is implemented on the Pytorch framework, and stochastic gradient descent (SGD) is applied for end-to-end training. We set the initial learning rate of layers before Pool5 in the master branch
as 0.0002, the final score layer as 0.005, and all other layers as 0.001. 
All those learning rates are decayed by a factor of 0.9 in every 50,000 iterations. A momentum of 0.9 and weight decay of 0.0005 are also applied. The network is continually trained %on a Nvidia Titan X Pascal GPU 
with a batch size of 100 until the loss does not further decrease.
 
%=================================================
\subsection{Additional one view data ??}
\label{ssec:oneview}

Possibility to add additional set of one view ??

